H2:Towards Efficient Large-Scale LLM Training on Hyper-Heterogeneous Cluster over 1,000 Chips

Recent advancements in large language models (LLMs) necessitate extensive computational resources, prompting the use of diverse hardware accelerators from multiple vendors. However, traditional distributed training frameworks struggle to efficiently utilize hyper-heterogeneous clusters comprising thousands of chips due to significant disparities in software stacks, operator implementations, communication libraries, and hardware capabilities. To address these challenges, we propose H2, which stands for HyperHetero and is a systematic framework enabling efficient training of LLMs on clusters with over 1,000 heterogeneous chips. H2 incorporates DiTorch, a unified PyTorch-compatible interface ensuring program consistency across chips, and DiComm, a device-direct RDMA communication library optimized for heterogeneous environments. Furthermore, we introduce HeteroPP with HeteroAuto, an adaptive pipeline parallelism strategy that dynamically balances computational load, memory limitations, and communication overhead. Evaluations on a 100-billion-parameter LLM demonstrate that our approach consistently achieves a superlinear speedup, outperforming baseline homogeneous training solutions by up to 16.37% in our experiments. These findings validate the feasibility and efficiency of hyper-heterogeneous training at unprecedented scales.

==> content/sec-8.tex <==
\section{Conclusion}
In this paper, we propose a unified framework H2 for efficient large language model training on hyper-heter-ogeneous clusters comprising over 1,000 chips with diverse architectures and software stacks. By integrating DiTorch and DiComm to unify the programming interface and communication library, our approach overcomes the challenges related to operator and communication isolation. In addition, the HeteroPP framework, together with the HeteroAuto automatic strategy search, dynamically optimizes parallelism configurations based on rigorous cost modeling and hardware profiling. Moreover, our topology-aware activation resharding strategy and fine-grained computation-communication overlapping minimizes cross-node data transfer delays, further improving overall performance. Experimental results on a 100B-parameter model demonstrate that our solution achieves a superlinear speedup compared to traditional homogeneous methods by effectively balancing computational loads, memory disparities, and communication overhead.

% In this paper, we introduce H2, a unified framework for efficiently training large language models on hyper-heterogeneous clusters comprising over 1,000 chips with diverse architectures and software stacks. By merging DiTorch and DiComm into a standardized programming and communication library, our approach effectively addresses software, operator and communication isolation issues. Furthermore, the HeteroPP framework, combined with HeteroAuto's automatic strategy search, dynamically refines parallelism configurations through rigorous cost modeling and hardware profiling. Additionally, our topology-aware activation resharding and fine-grained computation-communication overlapping substantially reduce cross-node data transfer delays, thereby enhancing overall performance. Experiments on a 100B-parameter model demonstrate that our solution achieves superlinear speedup over traditional homogeneous methods by balancing computational loads, memory disparities, and communication overhead.

